Generating Probabilities From Numerical Weather Forecasts by Logistic Regression

Logistic models are studied as a tool to convert output from numerical weather forecasting systems (deterministic and ensemble) into probability forecasts for binary events. A logistic model obtains by putting the logarithmic odds ratio equal to a linear combination of the inputs. As any statistical model, logistic models will suffer from over-fitting if the number of inputs is comparable to the number of forecast instances. Computational approaches to avoid over-fitting by regularisation are discussed, and efficient approaches for model assessment and selection are presented. A logit version of the so called lasso, which is originally a linear tool, is discussed. In lasso models, less important inputs are identified and discarded, thereby providing an efficient and automatic model reduction procedure. For this reason, lasso models are particularly appealing for diagnostic purposes.

==> apx_aic.tex <==
\section{The AIC}
% 
\label{apx:aic}
% 
In this appendix, an explicit form of the optimism $\delta$ in Equation~\ref{equ:6.105} is derived. 
% 
Both the Ignorance and the Brier score will be considered. 
% 
Furthermore, for the Ignorance the optimism will be interpreted in terms of the degrees of freedom of the model.
% 
That is, I will give a detailed derivation of Equation~\eqref{equ:6.160}.
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%Elsewhere
% 
The leave--one--out error will in general be larger than $R(\hat{\beta})$.
%
We now want to interprete the difference in terms of effective degrees of freedom of the model. 
% 
% 
Define $\delta$ by
% 
\beq{equ:6.105}
R_{\mbox{\tiny loo}}(\lambda) = R(\hat{\beta}) + \frac{\delta}{N},
\eeq
% 
It can be shown (see Appendix~\ref{apx:aic}) that for the Ignorance $\delta := \mbox{tr} \left(\mtr{L}_1 \mtr{L}_2^{-1}\right)$, with
% 
\begin{eqnarray}
\label{equ:6.110}
\left( \mtr{L}_1 \right)_{ij} & := & \frac{1}{N} \sum_m x^{(i)}_m x^{(j)}_m \hat{d}_m^2\\
\label{equ:6.115}
\mtr{L}_2 & := & \frac{1}{N} \mtr{X}^t \hat{\mtr{W}} \mtr{X} + \Lambda.
\end{eqnarray}
%
% 
To see why $\delta$ can be interpreted as the effective degrees of freedom of the model, we assume that to a high degree of accuracy, $g(X \hat{\beta}^t) = \pi(X)$.
%
Consequently, $\Ex \left[ (Y - g)^2 | X \right] = g (1 - g)$.
% 
For the Ignorance, $\mtr{d}$ and $\mtr{W}$ are given by Equation~\eqref{equ:6.55}. 
% 
Now, for $N$ large, 
\beq{equ:6.120}
\mtr{L}_1
\cong \Ex \left[ (g - Y)^2 X^t X \right]
= \Ex \left[ \Ex[(g - Y)^2|X] \*  X^t X \right]
= \Ex \left[ g(1-g) X^t X \right]
\eeq
% 
and
% 
\beq{equ:6.130}
\mtr{L}_2
\cong \Ex \left[g(1-g)  X^t X \right]  + \Lambda.
\eeq
% 
% 
Letting $ s_i, i = 1 \ldots d+1$ be the eigenvalues of $\Ex \left[ g(1-g) X^t X \right]$, we obtain after some calculations
% 
% 
\beq{equ:6.160}
\delta := \mbox{tr} \left( \mtr{L}_1 \mtr{L}_2^{-1} \right) = \sum_k \frac{s_k}{s_k + \lambda} + f(\lambda).
\eeq
% 
Here $f(\lambda) \in [0, 1]$ with $f(\lambda) = O(\lambda)$ for small $\lambda$ and $f(\lambda) \to 1$ for $\lambda \to \infty$.
% 
All in all, we get that $\delta \cong d + 1 - O(\lambda) $ for small $\lambda$ and $\delta \to 1 $ for large $\lambda$, where $d$ is the number of parameters in the model (not counting the intercept).
% 
If we interprete $\delta$ as the number of effective degrees of freedom of the model, we obtain the reassuring conclusion that for vanishing penalty the model has $d+1$ effective degrees of freedom, while for increasing penalty the number of effective degrees of freedom reduces to~$1$, owing to the fact that no penalty was imposed on the intercept $\beta_0$.
%

%
Equation~\eqref{equ:6.105} is a version of Akaike's information criterion (AIC)~\cite{hastie01}, which is given by
% 
% 
\beq{equ:6.190}
\mbox{AIC} := 2 R(\hat{\beta}) + 2 \* \frac{\delta}{N}.
\eeq
% 
The AIC is asymptotically equal to twice the expected Ignorance $\Ex \left[ S(g(X\hat{\beta}^t), Y)\right]$, where the expectation runs over the training set (and hence over $\hat{\beta}$) and over a new target~$Y$ (not in the training set).
%
It is possible to use the AIC directly as a criterion for determining the regularisation parameter.
% 
Although AIC and leave--one--out error are asymptotically the same, the two quantities can differ somewhat for very small sample sizes. 
% 
In this situation we found that a direct calculation of the leave--one--out error Equation~\eqref{equ:6.90} with the approximation~\eqref{equ:6.100} gives better results. 
%
% 
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

